A bright millisecond radio burst of extragalactic origin

Pulsar surveys offer one of the few opportunities to monitor even a small fraction (~0.00001) of the radio sky for impulsive burst-like events with millisecond durations. In analysis of archival survey data, we have discovered a 30-Jy dispersed burst of duration <5 ms located three degrees from the Small Magellanic Cloud. The burst properties argue against a physical association with our Galaxy or the Small Magellanic Cloud. Current models for the free electron content in the Universe imply a distance to the burst of <1 Gpc No further bursts are seen in 90-hr of additional observations, implying that it was a singular event such as a supernova or coalescence of relativistic objects. Hundreds of similar events could occur every day and act as insightful cosmological probes.

==> abstract <==
Pulsar surveys offer one of the few opportunities to monitor even a
small fraction ($\sim 10^{-5}$) of the radio sky for impulsive
burst-like events with millisecond durations. In analysis of archival
survey data, we have discovered a 30-Jy dispersed burst of duration
$<5$~ms located three degrees from the Small Magellanic Cloud. The
burst properties argue against a physical association with our Galaxy
or the Small Magellanic Cloud. Current models for the free electron
content in the Universe imply the burst is $<1$~Gpc distant. No
further bursts are seen in 90-hr of additional observations, implying
that it was a singular event such as a supernova or coalescence of
relativistic objects. Hundreds of similar events could occur every day
and act as insightful cosmological probes.

